Completeness for Game Logic

Game logic was introduced by Rohit Parikh in the 1980s as a generalisation of propositional dynamic logic (PDL) for reasoning about outcomes that players can force in determined 2-player games. Semantically, the generalisation from programs to games is mirrored by moving from Kripke models to monotone neighbourhood models. Parikh proposed a natural PDL-style Hilbert system which was easily proved to be sound, but its completeness has thus far remained an open problem. In this paper, we introduce a cut-free sequent calculus for game logic, and two cut-free sequent calculi that manipulate annotated formulas, one for game logic and one for the monotone mu-calculus, the variant of the polymodal mu-calculus where the semantics is given by monotone neighbourhood models instead of Kripke structures. We show these systems are sound and complete, and that completeness of Parikh's axiomatization follows. Our approach builds on recent ideas and results by Afshari & Leigh (LICS 2017) in that we obtain completeness via a sequence of proof transformations between the systems. A crucial ingredient is a validity-preserving translation from game logic to the monotone mu-calculus.

==> GL-abstract.tex <==
\begin{abstract}
Game logic was introduced by Rohit Parikh in the 1980s as a generalisation of 
propositional dynamic logic (PDL) for reasoning about 
outcomes that players can force in determined 2-player games.
%Where PDL is used to reason about outcomes of programs, game logic is used to
%reason about outcomes that players can force in determined 2-player games.
%These games are built from atomic games and various PDL-like game constructs. 
Semantically, the generalisation from programs to games is mirrored by moving from Kripke
models to monotone neighbourhood models.
%
Parikh proposed a natural PDL-style Hilbert system which was
easily proved to be sound, but its completeness has thus
far remained an open problem.

In this paper, we introduce a cut-free sequent calculus for game logic,
and two cut-free sequent calculi that manipulate annotated formulas, one
for game logic and one for the monotone $\mu$-calculus, the variant of
the polymodal $\mu$-calculus where the semantics is given by monotone
neighbourhood models instead of Kripke structures.
%The first system has an explicit induction rule and deep inference rules.
%The other two manipulates annotated formulas and constructs
%circular proofs in which infinite proof-branches
%are constrained by unfolding of greatest fixpoint formulas.  
We show these systems are sound and complete, and that
completeness of Parikh's axiomatization follows.
%
Our approach builds on recent ideas and results by Afshari \& Leigh (LICS 2017)
%who developed cut-free sequent calculi for the normal $\mu$-calculus.
in that we obtain completeness via a sequence of proof transformations
between the systems.   
A crucial ingredient is a validity-preserving translation from game logic to the 
monotone $\mu$-calculus.
% The key observation is that Kozen's context rule can be formulated in the 
% language of game logic.
\end{abstract}



==> ovw-diagram.tex <==
Let $\langNormAnn$ be annotated game logic formulas.

\[\xymatrix{
  \HilbP & \HilbFull & \GLms & \CloG & \CloM & \Clo
  \\
  \langPar & \langFull & \langNorm & \langNormAnn & \langMAnn & \langBimodAnn
}\]


==> sec-2d.tex <==
%\subsection{From \GLms  to \HilbP }\label{sec:G-to-HilbP}
% We don't need separate subsection anymore

The following theorem states the transformation results
between $\GLms$ and $\HilbP$ that are needed for proving
Theorem~\ref{thm:compGLms}. The proof of Theorem~\ref{thm:compGLms}
will be outlined in Section~\ref{sec:s-c}.

\begin{theorem}
  \label{thm:GLms-to-HilbP}
  We have:
  \begin{enumerate}
    \item 
      For all $\phi \in \langPar$,
      if $\GLms \vdash \dnnf{\phi}$ then $\HilbP \vdash \phi$.  
    \item For all $\xi \in \langNorm$,
      if $\GLms \vdash \xi$ then $\HilbP \vdash \pari{\xi}$.  
  \end{enumerate}
\end{theorem}


